A Multi-solution Study on GDPR AI-enabled Completeness Checking of DPAs

Specifying legal requirements for software systems to ensure their compliance with the applicable regulations is a major concern to requirements engineering (RE). Personal data which is collected by an organization is often shared with other organizations to perform certain processing activities. In such cases, the General Data Protection Regulation (GDPR) requires issuing a data processing agreement (DPA) which regulates the processing and further ensures that personal data remains protected. Violating GDPR can lead to huge fines reaching to billions of Euros. Software systems involving personal data processing must adhere to the legal obligations stipulated in GDPR and outlined in DPAs. Requirements engineers can elicit from DPAs legal requirements for regulating the data processing activities in software systems. Checking the completeness of a DPA according to the GDPR provisions is therefore an essential prerequisite to ensure that the elicited requirements are complete. Analyzing DPAs entirely manually is time consuming and requires adequate legal expertise. In this paper, we propose an automation strategy to address the completeness checking of DPAs against GDPR. Specifically, we pursue ten alternative solutions which are enabled by different technologies, namely traditional machine learning, deep learning, language modeling, and few-shot learning. The goal of our work is to empirically examine how these different technologies fare in the legal domain. We computed F2 score on a set of 30 real DPAs. Our evaluation shows that best-performing solutions yield F2 score of 86.7% and 89.7% are based on pre-trained BERT and RoBERTa language models. Our analysis further shows that other alternative solutions based on deep learning (e.g., BiLSTM) and few-shot learning (e.g., SetFit) can achieve comparable accuracy, yet are more efficient to develop.

==> RQ2.1_results.tex <==
\begin{table}[]
\caption{Per requirement results of the best performing binary BERT models and multi-class RoBERTa models fine-tuned on augmented datasets \textbf{(RQ2)}.}
\label{tab:per_req_results_RQ2}
\resizebox{12cm}{!}{
\begin{tabular}{@{}c|cccccc|cccccc@{}}
\toprule
\multirow{2}{*}{\textbf{R}} & \multicolumn{6}{c|}{\textbf{Best MCC Model (RB)}}                                                          & \multicolumn{6}{c}{\textbf{Best BCC Model (B)}}                                                             \\ \cmidrule(l){2-13} 
& \textbf{RQ1}  & \textbf{BT}   & \textbf{SR}   & \textbf{NBM}  & \textbf{SSE}  & \textbf{4T}   & \textbf{RQ1}  & \textbf{BT}   & \textbf{SR}   & \textbf{NBM}  & \textbf{SSE}  & \textbf{4T}   \\ \midrule
PO1   & 85.1          &  87.6          & 87.6          & \textbf{89.5}          & 84.2          & \textbf{89.5} & 94.7          & 89.5          & \textbf{99.0} & 89.5          & 94.1          & 88.5          \\
PO2   & 78.3          & 78.3          & \textbf{82.4} & 72.3          & 77.4          & 56.3          & \textbf{77.4} & 61.0          & 61.7          & 72.3          & 73.2          & 56.3          \\
PO3   & \textbf{94.2} & \textbf{94.2} & 78.9          & 91.2          & 91.2          & 93.5          & 93.5          & \textbf{97.1} & 91.2          & 94.2          & 93.5          & \textbf{97.1} \\
PO4   & 95.2          & 84.6          & 93.2          & 90.2          & \textbf{96.8} & 92.3          & 88.7          & \textbf{95.2} & 0.0           & 84.6          & 90.9          & 93.8          \\
PO5   & \textbf{95.0} & \textbf{95.0} & 74.6          & 85.5          & 78.3          & \textbf{95.0} & \textbf{98.4} & 95.0          & 92.4          & 95.8          & 95.0          & 89.0          \\
PO6  & 71.4          & \textbf{84.2} & 43.2          & 78.9         & 80.6          & 76.9          & 61.8          & 73.0          & 76.1          & \textbf{88.5} & 58.1          & 80.6          \\
PO7   & \textbf{94.3} & 84.0          & 80.5          & 87.5          & 77.6          & 90.9          & 87.5          & \textbf{94.3} & 90.9          & \textbf{94.3} & 80.5          & 84.0          \\
PO8   & \textbf{41.7} & 0.0           & 0.0           & 0.0           & 0.0           & 0.0           & 0.0           & \textbf{50.0} & 0.0           & 41.7          & 38.5          & 0.0           \\
PO9   & 46.9 & 34.5          & 46.9 & \textbf{50.0}          & 46.9 & 46.9 & 46.9          & 33.3          & \textbf{60.6} & 55.6          & 45.5          & 46.9          \\
PO10  & 0.0           & 0.0           & 0.0           & 0.0           & 0.0           & 0.0           & 0.0           & 0.0           & \textbf{83.3} & 0.0           & 0.0           & 0.0           \\
PO11  & \textbf{85.1} & 73.7          & 76.1          & 56.2          & 71.4          & 78.9          & \textbf{85.1} & 0.0           & 75.3          & 80.6          & 71.4          & 76.5          \\
PO12                                  & 55.6          & \textbf{83.3} & 45.5          & \textbf{83.3} & 41.7          & 43.5          & 55.6          & 50.0          & 45.5          & 45.5          & \textbf{100}  & 45.5          \\
PO13                                  & \textbf{99.2} & \textbf{99.2} & 89.4          & \textbf{99.2} & \textbf{99.2} & \textbf{99.2} & 96.0          & 99.2          & \textbf{99.2} & 96.0          & \textbf{99.2} & 92.7          \\
PO14                                  & 90.9          & 74.3          & \textbf{96.2} & 89.7          & 89.7          & 90.9          & 90.9          & 85.5          & \textbf{96.2} & 84.4          & 89.7          & 90.9          \\
PO15                                  & \textbf{83.3} & 71.4          & 68.5          & 53.8          & 53.0          & 64.3          & 0.0           & 67.6          & \textbf{71.4} & 64.3          & 65.2          & 63.4          \\
PO16                                  & \textbf{91.3} & 90.0          & 85.0          & 67.7          & 76.5          & \textbf{91.3} & 63.2          & \textbf{96.2} & 80.8          & 92.2          & 89.1          & 92.2          \\
PO17                                  & \textbf{99.1} & \textbf{99.1} & 95.5          & 94.6          & \textbf{99.1} & 98.2          & \textbf{95.5} & \textbf{95.5} & \textbf{95.5} & 89.3          & 93.8          & 91.7          \\
PO18                                  & \textbf{94.1} & 93.0          & \textbf{94.1} & \textbf{94.1} & \textbf{94.1} & \textbf{94.1} & \textbf{93.0} & \textbf{93.0} & 88.2          & 89.3          & 94.1          & 92.0          \\
PO19                                  & 68.2          & 50.8          & 43.9          & 72.6          & 68.2          & \textbf{73.5} & 67.2          & 0.0           & \textbf{73.5} & 69.2          & 72.5          & \textbf{73.5} \\ \midrule
\textbf{Summary}                      & \textbf{87.8} & \textbf{84.5} & \textbf{78.7} & \textbf{82.0} & \textbf{81.9} & \textbf{85.2} & \textbf{81.6} & \textbf{79.9} & \textbf{82.3} & \textbf{85.3} & \textbf{84.1} & \textbf{83.5} \\ \bottomrule
\end{tabular}}
\begin{tablenotes}
\centering
     \item[] \textbf{*}Abbreviations: Multi-class Classification (MCC), Binary Class Classification (BCC), BERT (B), RoBERTa (RB), Back Translation (BT), Synonyms Replacement (SR), Noise-based Methods (NBMs), Similar Semantic Embeddings (SSE), 4 Techniques (4T).
\end{tablenotes}
\end{table}






% \begin{table}[]
% \caption{Per requirement results of the best performing binary BERT models of RQ1 and all BERT models fine-tuned on augmented datasets.}
% \label{tab:per_req_results_RQ2}
% \resizebox{12cm}{!}{
% \begin{tabular}{@{}ccccccc@{}}
% \toprule
% \textbf{Requirement} & \textbf{BERT (RQ1)} & \textbf{BERT (BT)} & \textbf{BERT (SR)} & \textbf{BERT (NBM)} & \textbf{BERT (SSE)} & \textbf{BERT (4T)} \\ \midrule
% PO1                  & 94.7                & 89.5               & \textbf{99.0}      & 89.5                & 94.1                & 88.5               \\
% PO2                  & \textbf{77.4}       & 61.0               & 61.7               & 72.3                & 73.2                & 56.3               \\
% PO3                  & 93.5                & \textbf{97.1}      & 91.2               & 94.2                & 93.5                & \textbf{97.1}      \\
% PO4                  & 88.7                & \textbf{95.2}      & 0.0                & 84.6                & 90.9                & 93.8               \\
% PO5                  & \textbf{98.4}       & 95.0               & 92.4               & 95.8                & 95.0                & 89.0               \\
% PO6                  & 61.8                & 73.0               & 76.1               & \textbf{88.5}       & 58.1                & 80.6               \\
% PO7                  & 87.5                & \textbf{94.3}      & 90.9               & \textbf{94.3}       & 80.5                & 84.0               \\
% PO8                  & 0.0                 & \textbf{50.0}      & 0.0                & 41.7                & 38.5                & 0.0                \\
% PO9                  & 46.9                & 33.3               & \textbf{60.6}      & 55.6                & 45.5                & 46.9               \\
% PO10                 & 0.0                 & 0.0                & \textbf{83.3}      & 0.0                 & 0.0                 & 0.0                \\
% PO11                 & \textbf{85.1}       & 0.0                & 75.3               & 80.6                & 71.4                & 76.5               \\
% PO12                 & 55.6                & 50.0               & 45.5               & 45.5                & \textbf{100}        & 45.5               \\
% PO13                 & 96.0                & 99.2               & \textbf{99.2}      & 96.0                & \textbf{99.2}       & 92.7               \\
% PO14                 & 90.9                & 85.5               & \textbf{96.2}      & 84.4                & 89.7                & 90.9               \\
% PO15                 & 0.0                 & 67.6               & \textbf{71.4}      & 64.3                & 65.2                & 63.4               \\
% PO16                 & 63.2                & \textbf{96.2}      & 80.8               & 92.2                & 89.1                & 92.2               \\
% PO17                 & \textbf{95.5}       & \textbf{95.5}      & \textbf{95.5}      & 89.3                & 93.8                & 91.7               \\
% PO18                 & \textbf{93.0}       & \textbf{93.0}      & 88.2               & 89.3                & 94.1                & 92.0               \\
% PO19                 & 67.2                & 0.0                & \textbf{73.5}      & 69.2                & 72.5                & \textbf{73.5}      \\ \midrule
% \textbf{Summary}     & \textbf{81.6}       & \textbf{79.9}      & \textbf{82.3}      & \textbf{85.3}       & \textbf{84.1}       & \textbf{83.5}      \\ \bottomrule
% \end{tabular}}
% \begin{tablenotes}
% \centering
%      \textbf{*Abbreviations:} Back Translation (BT), Synonyms Replacement (SR), Noise-based Methods (NBMs), Similar Semantic Embeddings (SSE), 4 Techniques (4T).
% \end{tablenotes}
% \end{table}

==> RQ3_results.tex <==

\begin{table*}[]
\caption{Results of RoBERTa and BERT fine-tuned on the balanced original and augmented datasets \textbf{(RQ3)}.}
\label{tab:results_RQ3}
\resizebox{12cm}{!}{
\begin{tabular}{@{}lcccc|cccc@{}}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{4}{c}{\textbf{Best MCC Model (RB)}}     & \multicolumn{4}{|c}{\textbf{Best BCC Model (B)}}    \\ \cmidrule(l){2-9} 
& \textbf{A} & \textbf{P} & \textbf{R} & \textbf{F$_2$} & \textbf{A} &  \textbf{P} & \textbf{R} & \textbf{F$_2$}  \\ \midrule
RQ1 (FD)  & 83.5          & 80.5          & 89.8          & 87.8           & 80.9                              & 81.4          & 81.6          & 81.6           \\ \midrule
RQ2 (FAD) & 83.5          & 80.5          & 89.8          & 87.8           & 78.6                              & 74.7          & 88.4          & 85.3           \\ \midrule
RUS  & \textbf{76.7} & \textbf{69.8} & \textbf{96.6} & \textbf{89.7}  & 54.7          & 53.3          & 99.7          & 84.9           \\
ROS  & 79.1          & 74.2          & 91.2          & 87.2           & \textbf{79.5} & \textbf{75.1} & \textbf{90.1} & \textbf{86.7}  \\
RUOS   & 82.5          & 85.0          & 81.7          & 82.3           & 63.0          & 58.4          & 98.3          & 86.5           \\ \midrule
BT-RUS  & 77.5          & 71.3          & 94.6          & 88.8           & 58.1                              & 55.2          & 99.3          & 85.6           \\
SR-RUS   & 80.4          & 75.4          & 91.8          & 88.0           & 59.3                              & 56.0          & 99.0          & 85.8           \\
NBM-RUS  & 78.4          & 75.7          & 85.7          & 83.5           & 60.7                              & 56.9          & 98.3          & 85.8           \\
SSE-RUS  & 79.3          & 79.7          & 80.3          & 80.2           & 60.7                              & 56.9          & 98.3          & 85.8           \\
4T-RUS  & 78.4          & 74.9          & 87.4          & 84.6           & 61.6                              & 57.4          & 99.0          & 86.5           \\ \bottomrule

\end{tabular}}
\begin{tablenotes}
\centering
     \item[]\textbf{*}Abbreviations: Multi-class Classification (MCC), Binary Class Classification (BCC),  Precision (P), Recall (R), F$_2$-score (F$_2$), Accuracy (A), RoBERTa (RB), BERT (B), Full Dataset (FD), Full Augmented Dataset (FAD), Random Undersampling (RUS), Random Oversampling (ROS), Random Under-Oversampling (UOS), Back Translation (BT), Synonyms Replacement (SR), Noise-based Methods (NBMs), Similar Semantic Embeddings (SSE), 4 Techniques (4T).
\end{tablenotes}
\end{table*}



% \begin{table*}[]
% \caption{Results of RoBERTa and BERT fine-tuned on the balanced original and augmented datasets \textbf{(RQ3)}.}
% \label{tab:results_RQ3}
% \resizebox{12cm}{!}{
% \begin{tabular}{@{}lccc|ccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c}{\textbf{Best MCC Model (RB)}}     & \multicolumn{3}{|c}{\textbf{Best BCC Model (B)}}    \\ \cmidrule(l){2-7} 
% & \textbf{P} & \textbf{R} & \textbf{F$_2$} & \textbf{P} & \textbf{R} & \textbf{F$_2$} \\ \midrule
% RQ1 (FD)     & 80.5               & 89.8            & 87.8              & 81.4               & 81.6            & 81.6              \\ \midrule
% RQ2 (FAD)                              & 80.5               & 89.8            & 87.8              & 74.7               & 88.4            & 85.3              \\ \midrule
% RUS                               & \textbf{69.8}      & \textbf{96.6}   & \textbf{89.7}     & 53.3               & 99.7            & 84.9              \\
% ROS                               & 74.2               & 91.2            & 87.2              & \textbf{75.1}      & \textbf{90.1}   & \textbf{86.7}     \\
% RUOS                              & 81.4               & 86.1            & 85.1              & 58.4               & 98.3            & 86.5              \\ \midrule
% BT-RUS      & 71.3               & 94.6            & 88.8              & 55.2               & 99.3            & 85.6              \\
% SR-RUS      & 75.4               & 91.8            & 88.0              & 56.0               & 99.0            & 85.8              \\
% NBM-RUS     & 75.7               & 85.7            & 83.5              & 56.9               & 98.3            & 85.8              \\
% SSE-RUS     & 79.7               & 80.3            & 80.2              & 56.9               & 98.3            & 85.8              \\
% 4T-RUS      & 74.9               & 87.4            & 84.6              & 57.4               & 99.0            & 86.5              \\ \bottomrule
% \end{tabular}}
% \begin{tablenotes}
% \centering
%      \item[]\textbf{*}Abbreviations: Multi-class Classification (MCC), Binary Class Classification (BCC),  Precision (P), Recall (R), F$_2$-score (F$_2$), RoBERTa (RB), BERT (B), Full Dataset (FD), Full Augmented Dataset (FAD), Random Undersampling (RUS), Random Oversampling (ROS), Random Under-Oversampling (UOS), Back Translation (BT), Synonyms Replacement (SR), Noise-based Methods (NBMs), Similar Semantic Embeddings (SSE), 4 Techniques (4T).
% \end{tablenotes}
% \end{table*}




% \begin{table*}[]
% \centering
% \caption{Results of RoBERTa and BERT fine-tuned on the various balanced datasets.}
% \label{tab:results_RQ3}
% \resizebox{12cm}{!}{
% \begin{tabular}{@{}lccc|ccc@{}}
% \toprule
% \multirow{2}{*}{Dataset} & \multicolumn{3}{c}{\textbf{Best MCC Model (RoBERTa)}}  & \multicolumn{3}{|c}{\textbf{Best Binary Model (BERT)}}       \\ \cmidrule(l){2-7} 
%     &  \textbf{Precision} & \textbf{Recall} & \textbf{F$_2$-score} & \textbf{Precision} & \textbf{Recall} & \textbf{F$_2$-score} \\ \midrule
%     RQ1   & 80.5  & 89.8  & 87.8   & 81.4  & 81.6  & 81.6  \\ \midrule
%     RUS  & \textbf{69.8} & \textbf{96.6}   & \textbf{89.7}     & 53.3               & 99.7  & 84.9 \\
%     ROS                   & 74.2               & 91.2            & 87.2              & \textbf{75.1}               & \textbf{90.1}    & \textbf{86.7}              \\
%     RUOS                  & 81.4               & 86.1            & 85.1              & 58.4 & 98.3            & 86.5     \\ \bottomrule
% \end{tabular}}
% \begin{tablenotes}
% \centering
%      \textbf{*Abbreviations:} Multi-class Classification (MCC), Random Undersampling (RUS), Random Oversampling (ROS), Random Under-Oversampling (UOS).
% \end{tablenotes}
% \end{table*}



==> RQ4_results.tex <==


\begin{table}[!t]
\centering
\caption{Execution time of the alternative solutions from the perspective of developers and end-users.}
\label{tab:RQ4_results}
\begin{tabular}{@{}lcc|cc@{}}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{2}{c|}{\textbf{Multi-class Classification}} & \multicolumn{2}{c}{\textbf{Binary Classification}} \\ \cmidrule(l){2-5} 
\multicolumn{1}{c}{} & \textbf{\begin{tabular}[c]{@{}c@{}}Developer's \\ Perspective \\ (min)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}End-user's\\ Perspective \\ (ms)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Developer's \\ Perspective \\ (min)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}End-user's\\ Perspective \\ (ms)\end{tabular}} \\ \cmidrule(r){1-5}
ALBERT    & 27       &    91      &  484    &  1364   \\
BERT      & 31       &    91      &  448    &  1390  \\
Legal-BERT  & 42     &    92      &  439    &  1660   \\
RoBERTa     & 24     &    92      &  489    &  1557   \\
BiLSTM      & 7      &    4.4     &  227    &   93   \\
MLP         &  3     &    4       &  46     &   71  \\
SVM      &    2      &    4.4     &  18     &   71   \\
RF       &    2      &    4       &  22     &   71   \\
LR      &     2      &    4       &  18     &   80       \\ 
SETFIT  &   51       &   3        &  971    &   98\\ \bottomrule
\end{tabular}
\end{table}




==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
In this section, we discuss the practical implications and applications of the best performing alternative solution RoBERTa (multi-class) for compliance checking of DPA against GDPR. 
  


\subsection{Practical Implications} 
In this subsection we discuss how can the best alternative solution RoBERTa (multi-class) help a human analysts in checking compliance of a DPA against GDPR. As mentioned in Section~\ref{subsec:RQ3} that the best alternative solution achieves an average F$_2$-score of 89.7\%. In this study we favor recall over precision because an unsatisfactory recall may miss \textbf{satisfied} requirements in the DPA. In such a case, a human analyst would need to read the whole DPA to identify the missing requirements which reduces the application of our model. Our model will help the human analyst when it achieves higher recall means produces less FNs. We observed that RoBERTa (multi-class) produces 10 FNs. We analyze these cases to understand the root causes behind them. In the following subsection we discuss the causes of the FNs along with examples from the \textsc{testing set}. 

\paragraph{In complete sentences} 1 FN is produce by the model due to this error. As mentioned in Section~\ref{sec:automated_complaince_checking} that the DPA text is tokenized into sentences using our NLP pipeline. DPA text most often contains bulleted text. Our NLP pipeline split the bulleted text into various sentences which are individually given as input to the model. The splitting of bulleted text leads to the loss of context as illustrated in the following example: ``While working as a processor on behalf of a controller, the processor shall:
\begin{itemize}
    \item only process personal data on in accordance with controller's written instructions;
    \item ensure that persons authorized to process the Personal Data in the provision of the Services keep such Personal Data confidential;  
    \item not disclose Personal Data to any third parties without controller’s prior consent, except as required by law or permitted by the Agreement.'' 
\end{itemize}
The above example is split into four sentences by our NLP pipeline which make the sentences grammatically incomplete. Our model could have identified the first two sentences together as satisfying requirement PO3 and the first and the third sentences together as PO5. However, these sentences individually are semantically quite different from each other. Therefore the model cannot identify them as satisfied sentences. 

\paragraph{Long verbose sentences} 4 FNs are produced due to this error. The DPA sentences are often long and contain text which is not relevant to requirements they are satisfying. An example of such a sentence is: ``controller hereby agrees (i) to limit any inspection to the extent reasonably necessary to confirm such compliance, (ii) to enter into a confidentiality agreement (in a form reasonably acceptable to controller) in respect of any information that its representative may incidentally be provided access to while carrying out an inspection, (iii) to ensure that controller's personnel shall comply with all processor's security policies at the relevant processor locations and shall always be accompanied by a representative of processor, and (iv) to indemnify processor against any loss or damage to processor arising from the negligence of controller's personnel whilst such personnel are carrying out the activities described in this clause.'' The semantics of such long sentences are hard to understand and the model fails to identify them correctly. 

The both the above errors can be handled by defining heuristics to identify and paraphrase the itemized lists or filter out noisy content from DPA. 

\paragraph{Similar Requirements} 4 FNs produced by the model is attributed to the similarity of the requirements. As mentioned in Section~\ref{subsec:RQ1} that some requirements are very similar to each other as they either belong to the same GDPR article e.g., P015 and PO16 belongs to Article 28(3) or they describe the same subject e.g.,  data security or controller's assistance etc. These requirements often share similar textual content due to which the model may confuse them. For example the sentence ``make available to controller all information necessary to demonstrate compliance with the obligations set out in this Clause and allow for and contribute to audits, including inspections, conducted by controller or another auditor mandated by it.'' is annotated as PO16 in the \textsc{testing set} but the model predict it as PO15, hence leading to a FN. The main reason could be the similarity of textual content of the sentence to both the requirements. 

\paragraph{References to Sections} Another cause behind the FNs is the references in the DPA sentences to other sections of the DPA. 1 FN occurred due to this error. An example of the DPA sentence containing references to sections is ``The Processor shall process the Personal data described in this Section 2 for the purpose of providing the Services set out in Schedule 2.1.1 of the Agreement, in particular:''. This sentence is annotated as PO2 in the \textsc{testing set} by the annotators. A human analyst can check the specified section to verify that the section is about the requirement PO2. However, the sentence itself does not provide all the information needed for the model to predict it as PO2. 
  

\subsection{Applications of the proposed solution}
The solution proposed in this study applies to both real businesses and software development. As most businesses are now data-driven and share their data somehow for processing with other organizations. They are bound to sign a DPA with the organization processing data on their behalf. Such businesses can use the proposed solution to check the compliance of their DPAs against GDPR requirements. Particularly legal firms, which provide their services of compliance checking to other organizations, can get benefits from our solution. As mentioned in Section~\ref{subsec:RQ4} the proposed solution can process an average size DPA just in $\approx20$ seconds hence saving both the time and effort required to read the whole DPA.

Software systems that involve sharing and processing of personal data are subject to compliance with GDPR. While developing such software systems, requirement engineers are required to extract compliance-related requirements from the legal documents (e.g. DPA) to ensure that all the processes comply with the GDPR. As requirement engineers have little knowledge of the legal domain hence it is hard for them to extract compliance requirements from legal documents. Our solution can help requirement engineers to extract requirements from DPAs to develop GDPR-compliant software.


==> hyper_para_tables.tex <==
\begin{table}[]
\centering
\caption{Best hyper parameters for LMs in Multi-class classification.}
\label{tab:hp_mcc}
\begin{tabular}{@{}|l|c|c|c|c|@{}}
\toprule
Model       & Batch Size & Epochs & Learning Rate \\ \midrule
ALBERT   & 32         & 10     & 2e-05         \\ \midrule
BERT          & 64         & 20     & 3e-05         \\ \midrule
Legal-BERT   & 32         & 20     & 2e-05         \\ \midrule
RoBERTa    & 64         & 10     & 2e-05         \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{Best hyper parameters for LMs in binary class classification.}
\label{tab:hp_binary}
\begin{tabular}{@{}|l|c|c|c|c|@{}}
\toprule
Model     & Batch Size & Epochs & Learning Rate \\ \midrule
ALBERT       & 64         & 10     & 2e-05         \\ \midrule
BERT          & 64         & 20     & 3e-05         \\ \midrule
Legal-BERT    & 32         & 20     & 2e-05         \\ \midrule
RoBERTa      & 64         & 20     & 2e-05         \\ \bottomrule
\end{tabular}
\end{table}



\begin{table}[]
\centering
\caption{Best hyper parameters for ML in Multi-class classification.}
\label{tab:hp_binary}
\begin{tabular}{@{}|l|c|c|c|c|@{}}
\toprule
Model     & Batch Size & Epochs & Learning Rate \\ \midrule
BiLSTM      & 128         & 50     & 0.01         \\ \midrule
MLP          & 32         & 100     & 5e-05         \\ \bottomrule
\end{tabular}
\end{table}

==> imbalance-table.tex <==
\begin{table*}
\caption{Summary of Data Imbalance Handling Strategies.}\label{tab: io}
%\vspace*{-.75em}
%\footnotesize
  \centering
\begin{threeparttable}[t]
 \begin{tabularx}{\textwidth} {@{} p{0.08\textwidth} | @{\hskip 0.5em}  X}
    \toprule
     Dataset & Description (\textbf{D}), Strategy (\textbf{G}), Average Proportion of Classes (\textbf{P}) \\ 
         \midrule
     \centering $\tau$ & Let $N^+$ denotes the number of positive examples, and $N_j^+$ denotes the number of positive examples for a given provision $p_j$
     \\
     &\textit{Multi-class classification}:  The number of classes $=$ 20; corresponding to the provisions $\{p_1 \ldots p_{19}\}$ and \textit{other} representing the  sentences that do not satisfy any provision. \textbf{P}:   \\
     \midrule
     \centering $\tau$+\textit{RO} & \textbf{D}:  Original training dataset with random oversampling. \textit{Binary classification}:  \textbf{G}:  For each $p_j$, the positive examples are randomly oversampled to become equal to the negative examples. \textbf{P}:  \colorbox{green!25}{50\%}: \colorbox{red!25}{50\%}\\ 
     & \textit{Multi-class classification}:  \textbf{G}:  All provisions are randomly oversampled to become equal to the \textit{other} class. %\textbf{P}:  \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{red!25}{10\%} 
     \\
     \midrule
     \centering $\tau$+\textit{RO} +\textit{RU} & \textbf{D}: Original training dataset with random undersampling. \textit{Binary classification}: \textbf{G}: For each $p_j$, the negative examples are randomly undersampled to become equal to the positive examples. \\
     &\textit{Multi-class classification}: \textbf{G}:  \\
     \midrule
     \centering $\tau$+\textit{RU} & \textbf{D}: Original training dataset with random undersampling. \textit{Binary classification}: \textbf{G}: For each $p_j$, the negative examples are randomly undersampled to become equal to the positive examples. \\
     &\textit{Multi-class classification}: \textbf{G}: The \textit{other} class is randomly undersampled to the \\
     \midrule
        \bottomrule
     
 \end{tabularx}
  \begin{tablenotes}
     \vspace*{.5em}
     \it\item[*] Value 
     \end{tablenotes}
  \end{threeparttable}
 % \vspace*{-.5em}
\end{table*}

\iffalse \begin{table*}
\caption{Summary of Data Imbalance Handling Strategies.}\label{tab: io}
%\vspace*{-.75em}
%\footnotesize
  \centering
\begin{threeparttable}[t]
 \begin{tabularx}{\textwidth} {@{} p{0.08\textwidth} | @{\hskip 0.5em}  X}
    \toprule
     Dataset & Description (\textbf{D}), Strategy (\textbf{G}), Average Proportion of Classes (\textbf{P}) \\ 
         \midrule
     \centering $\tau$ & \textbf{D}:  Original training dataset. \textit{Binary classification}:  For each $p_j$, positive examples are all sentences that satisfy $p_j$. Conversely, negative examples are all sentences that do not satisfy $p_j$. \textbf{P}:  \colorbox{green!25}{12\%}: \colorbox{red!25}{88\%}. \\
     &\textit{Multi-class classification}:  The number of classes $=$ 20; corresponding to the provisions $\{p_1 \ldots p_{19}\}$ and \textit{other} representing the  sentences that do not satisfy any provision. \textbf{P}:   \\
     \midrule
     \centering $\tau$+\textit{RO} & \textbf{D}:  Original training dataset with random oversampling. \textit{Binary classification}:  \textbf{G}:  For each $p_j$, the positive examples are randomly oversampled to become equal to the negative examples. \textbf{P}:  \colorbox{green!25}{50\%}: \colorbox{red!25}{50\%}\\ 
     & \textit{Multi-class classification}:  \textbf{G}:  All provisions are randomly oversampled to become equal to the \textit{other} class. %\textbf{P}:  \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{grey!25}{10\%}: \colorbox{red!25}{10\%} 
     \\
     \midrule
     \centering $\tau$+\textit{RO} +\textit{RU} & \textbf{D}: Original training dataset with random undersampling. \textit{Binary classification}: \textbf{G}: For each $p_j$, the negative examples are randomly undersampled to become equal to the positive examples. \\
     &\textit{Multi-class classification}: \textbf{G}:  \\
     \midrule
     \centering $\tau$+\textit{RU} & \textbf{D}: Original training dataset with random undersampling. \textit{Binary classification}: \textbf{G}: For each $p_j$, the negative examples are randomly undersampled to become equal to the positive examples. \\
     &\textit{Multi-class classification}: \textbf{G}: The \textit{other} class is randomly undersampled to the \\
     \midrule
        \bottomrule
     
 \end{tabularx}
  \begin{tablenotes}
     \vspace*{.5em}
     \it\item[*] Value 
     \end{tablenotes}
  \end{threeparttable}
 % \vspace*{-.5em}
\end{table*}

\fi

==> o_eval.tex <==
\iffalse
The dataset used in this study is comprised of 169 DPAs where 100 DPAs have been provided by our collaborating partners and the rest have been collected from online resources. To manually annotate the sentences in the DPAs that comply with GDPR requirements, we used the 45 GDPR requirements devised by Amaral et al.~\cite{amaral:21}. Three third-party annotators were given the DPAs to read through and check for compliance against GDPR requirements.
%Table \ref{} illustrates statistical data of the dataset. 
% A two-step procedure has been used to manually annotate the sentences in the DPAs that comply with the GDPR requirements.
% In the first step, 24 DPAs have been manually analyzed for compliance with the GDPR requirements by three researchers. Specifically, every single sentence of the DPA is analyzed and annotated with the requirement(s) it is satisfying. This annotation process was completed in two working weeks followed by various joint sessions where conflicts and observations were discussed. After the conflicts are carefully resolved, we discussed with our collaborating partners the sentences that were not straightforward. We had four sessions with the legal experts where the conflicts and doubts were discussed and resolved. During these sessions, we acquired knowledge about compliance checking and developed annotation guidelines for the second step.
% In the second step, the remaining 145 DPAs were read through and checked for compliance against GDPR by three third-party annotators. 
All of the annotators are law students who underwent a half-day training on compliance according to GDPR. The DPAs to be annotated and the list of GDPR requirements were shared with the annotators. The annotators were instructed to examine each sentence in the DPA and select all requirements that the sentence satisfies. The annotators completed their annotation task within three months. 
% This annotation process resulted in analyzing a total of 31,185 sentences, out of which 3387 are marked as satisfying at least one requirement under the \textit{processor's obligations} category, which is our focus here ($\approx$36\% of the total sentences satisfying any GDPR requirement).  


To measure the quality of the annotations, we computed the interrater agreement using Cohen’s Kappa ($\kappa$)~\cite{Cohen:60} on a subset (five DPAs) of the testing dataset. The average $\kappa$ value across pair-wise agreements for the annotations concerning \textit{processor's obligations} is 0.82, suggesting ``almost perfect agreement''~\cite{Viera:05}. We observe that achieving this high $\kappa$ value in our work is affected by the ample legal expertise of the annotators and the high comprehensibility of the requirements.


\paragraph{Dataset Distribution} As mentioned above our dataset consists of 169 DPAs and a total of 31,185 sentences. The distribution of the dataset is highly imbalanced as only 3,387 sentences ($\approx$11\%) satisfy one or more GDPR requirement(s) and the rest are other sentences, labeled in the dataset as `\textbf{Other}'. Besides, the distribution of the \textbf{satisfied} sentences in the dataset is also imbalanced as given in Table \ref{tab:reqs_dist}. 
The dataset is divided into a \textsc{training set}, containing 139 DPAs ($\approx70$\% of the dataset), and a \textsc{testing set} containing the rest of the 30 DPAs ($\approx30$\% of the dataset). The \textsc{training set} is further split into 80\% \textsc{training set} is used for training/fine-tuning of the models and 20\% \textsc{validation set} used for the validation during training/fine-tuning.
% The \textsc{validation set} (20\% of the train set) is used during training/fine-tuning to validate the models. 
Whereas the \textsc{testing set} is kept unseen to the training process and used only for the evaluation of the models. 


% \begin{figure} [t!]
% \centering
% \includegraphics[width=\textwidth]{figs/data_dist.pdf}
% % \vspace{-1em}
% \caption{Distribution of GDPR requirements in the dataset.}
% \label{fig:train_reqs_dist}
% % \vspace{-1.5em}
% \end{figure}

\subsection{Evaluation Metrics}
The models for compliance checking of the GDPR requirements are evaluated using \textit{precision (P)}, \textit{recall (R)}, and \textit{F$_2$-score} computed as \textit{P = TP / (TP + FP)}, \textit{R = TP / (TP + FN)}, and \textit{F$_2$-score = (5 * P * R) / (4 * P + R)} respectively. A \textit{true positive TP} is the case when a requirement is satisfied in the DPA, and the solution classify at least one sentence as the requirement. A \textit{false positive (FP)} is the case when a requirement is violated in the DPA, and the solution classify at least one sentence as the requirement. A \textit{false negative (FN)} is the case when a requirement is satisfied in the DPA, and the solution does not predict at least one sentence as the requirement. In this study we favor recall over precision, therefore we report F$_2$-score. In case of unsatisfactory recall, the model may not identify the \textbf{satisfied} requirements. 
The human analyst would need to read through the whole DPA to identify the requirements. Which reduces the usability of model in practice. On the other hand, unsatisfactory precision results in falsely identifying the `Other' sentences as \textbf{satisfied}. In such a case the human analyst can read through a set of sentences labeled by the model to verify whether they are correct.    
% \textcolor{red}{The recall of a model that identifies the processor's obligations is more important than its precision because missing a processor's obligation could have serious consequences for both the requirements engineer and legal experts e.g., non-compliance which in turn can lead to heavy fines. In addition, recall is particularly important when dealing with imbalanced datasets where one class is much more prevalent than the other. In such cases, a model that simply predicts the majority class for all instances can achieve high accuracy and precision, but its recall for the minority class may be very low, which is not desirable in our scenario.}

\subsection{Analysis Procedure}
The following subsections presents the hyper-parameter optimization used for the LLMs and ML models, methods used for the generation of augmented and balanced datasets.
\subsubsection{Hyperparameter Optimization}
\label{subsec:hyperparameters}
To get the best results out of all the models including the LLMs and the ML models in compliance checking of the DPA against GDPR, we have performed hyperparameter tuning. All the models are tuned to get the highest F$_2$-score for classifying the DPA sentences into the GDPR requirements. 
\paragraph{LLMs hyperparameter tuning} The LLMs have been optimized using a range of values for the three hyperparameters including batch size (32, 64, 128), epochs (10, 20), and learning rates (2e-05, 3e-05, 4e-05, 5e-05). We have used a dropout probability of 0.3. To optimize the models, recommendations in the relevant literature have been followed~\cite{hey:20,Sun:19}.The best hyper-parameters selected for the LMs in both the binary and multi-class classification task are given in the appendix \ref{sec:appendix_B}. 

\paragraph{ML models hyperparameters tuning} To optimize the classical machine learning models including SVM, logistic regression, and random forest, a range of values for hyperparameters associated with each model have been used. Grid Search \cite{pedregosa_scikit:11}  method of has been used to select the most optimal values for the models. 

Besides, we have optimized the two deep learning models a multi-layer perceptron and BiLSTM using the three hyper-parameters batch size (32, 64, 128), epochs (25, 50, 100), and learning rates (0.01, 0.0001). Recommendations from relevant literature has been followed to optimize the models~\cite{xu_bilstm:19}. The best-selected hyper-parameters for the ML model across both the classification tasks are given in the appendix \ref{sec:appendix_B}. 


\subsubsection{Augmented Data Generation}
\label{subsubsec:AD_generation}
To generate more annotated data in the \textsc{training set}, we have used various data augmention methods as explained in Section~\ref{subsubsec:data_aug}. The augmentation methods are applied to the \textbf{satisfied} sentences in the \textsc{training set} to generate the augmented data. The augmented data is then combined with the original \textsc{training set} to get the final training dataset. The following are the data augmentation methods used in this study.

\paragraph{Back Translation (BT)} In the BT method we have used two language translation models, i.e., French and German, to generate augmented sentences for all the \textbf{satisfied} sentences in the \textsc{training set}. The resulting dataset contains 5,742 augmented sentences. 

\paragraph{Synonym Replacement (SR)} In SR method, a single augmented sentence is generated per \textbf{satisfied} sentence in the \textsc{training set}. We have used two sources for SR such as WordNet and PPDB, therefore the resulting dataset contains augmented sentences double in size of the \textbf{satisfied} sentences.

\paragraph{Similar Semantic Embeddings (SSE)} In the SSE we have used three language models including BERT, RoBERTa, and ALBERT to generated augmented sentences. Each model is applied to the \textbf{satisfied} sentences in the \textsc{training set} to generated a single augmented sentence per \textbf{satisfied} sentence. The resulting augmented sentences are thrice in number (8,613) of the \textbf{satisfied} sentences. 

\paragraph{Noised-based methods (NBM)} In the NBM, we have used four different operations, as discussed in Section~\ref{subsec:DIHT}, to generate the augmented dataset. Each operation produces a single augmented sentence per \textbf{satisfied} sentence in the \textsc{training set}. The resulting augmented dataset contains 11,484 augmented sentences.

\subsubsection{Imbalance Handling}
\label{subsec:Imbalance_handling}
The data imbalance issue is handled using the data resampling methods as mentioned in Section~\ref{subsec:DIHT}. The following three data resampling have been used to produce balanced datasets.
\paragraph{Random Undersampling (RUS)} In the case of binary classification, the majority class is randomly undersampled to the minority class e.g. requirement PO1 has a total number of 187 instances in the \textsc{training set} as illustrated in Table~\ref{tab:reqs_dist}. A random sample of 187 sentences is randomly selected from the rest of the \textsc{training set} to balance the dataset. In the case of multi-class classification, the majority class `other' is undersampled to the most frequently occurred minority class `PO6' to get a balanced dataset.

\paragraph{Random Oversampling (RUS)}In case of binary classification, the minority class e.g., `PO1' is randomly oversampled to the majority class `other'. Similarly, in case of multi-class classification, all the minority classes e.g. PO1, PO2, etc. in the \textsc{training set} are oversampled to the majority class `other' to get a balanced dataset.

\paragraph{Random Under-oversampling (RUOS)} In this technique the \textsc{training set} is balanced in two steps: Firstly, the majority class `other' is undersampled to the most frequently occurred minority class `PO6'. Secondly, all the other minority classes e.g. PO1, PO2, etc. in \textsc{training set} are oversampled to the most frequently occurred class `PO6' to get a balanced dataset.

\fi




